Vector Bin-and-Cancel for MIMO Distributed Full-Duplex

In a multi-input multi-output (MIMO) full-duplex network, where an in-band full-duplex infrastruc- ture node communicates with two half-duplex mobiles supporting simultaneous up- and downlink flows, the inter-mobile interference between the up- and downlink mobiles limits the system performance. We study the impact of leveraging an out-of-band side-channel between mobiles in such network under different channel models. For time-invariant channels, we aim to characterize the generalized degrees- of-freedom (GDoF) of the side-channel assisted MIMO full-duplex network. For slow-fading channels, we focus on the diversity-multiplexing tradeoff (DMT) of the system with various assumptions as to the availability of channel state information at the transmitter (CSIT). The key to the optimal performance is a vector bin-and-cancel strategy leveraging Han-Kobayashi message splitting, which is shown to achieve the system capacity region to within a constant bit. We quantify how the side-channel improve the GDoF and DMT compared to a system without the extra orthogonal spectrum. The insights gained from our analysis reveal: i) the tradeoff between spatial resources from multiple antennas at different nodes and spectral resources of the side-channel, and ii) the interplay between the channel uncertainty at the transmitter and use of the side-channel.

==> Intro.tex <==
% !TEX root = JSACsidechannel.tex

\section{introduction}
%The readily accessible wireless devices with multi-radio interfaces allows the use of multiple wireless standards. Thus mobile nodes can access multiple orthogonal spectral bands simultaneously, which provides the opportunities to establish device-to-device~(D2D) wireless side channels when the mobile nodes are associated with cellular base station in the main channels. Such D2D wireless side channels can be leveraged to facilitate main channel cellular communication. Recent researches on full-duplex capable infrastructure node~\cite{Everett12Thesis} in short to medium ranges shows the feasibility of full-duplex wireless which greatly improve the spectral efficiency over its half-duplex counterpart, and opens new design opportunities for cellular wireless communication systems, such as small cells~\cite{Smallcell}.
%
%Consider the three-node network shown in Figure~\ref{fig.1}. A full-duplex capable base station~(BS)
%communicates with two half-duplex mobiles simultaneously to support one uplink~(UL) and one downlink~(DL) flow. One of the bottleneck in this network is the inter-node interference (INI) from UL mobile node to DL mobile node. In \cite{JingwenTWC}, we propose a \emph{distributed full-duplex architecture} as protocols for communication in side-channel assisted three-node network, and study how to leverage the D2D wireless side channel for interference management in such network with single transmit and receive antenna~(single-input single-output (SISO) channel).
%\begin{figure}[h!]
%  \centering
%%\flushleft
%%\flushright
%    \includegraphics[width=0.5\textwidth,trim = 60mm
%      50mm 60mm 40mm, clip]{../pic/topology.pdf}
%  \caption{\emph{MIMO three-node full-duplex network: inter-node interference becomes an important factor when the infrastructure node communicates with uplink and downlink mobile nodes simultaneously.}}
%\label{fig.1}
%\end{figure}
%Multiple-input multiple-output (MIMO) communication is well-known to improve the spectral efficiency and reliability upon single-antenna case. The diversity multiplexing tradeoff~(DMT), introduced in \cite{DMTTse}, captures both spectral efficiency and reliability of MIMO system in high signal-to-noise ratio~(SNR) limit. The DMT is also characterized for two-user interference channel~\cite{icdmt} and \cite{icdmt2} where each user can have different diversity and multiplexing gain requirement. In \cite{DMTMIMOZ}, the optimal, i,e., fundamental DMT is derived for MIMO Z-interference channel.
%The result of DMT is especially relevant in a slowly varying channel when the ergodic capacity can not be a meaningful metric.
%
%In this paper, we will study the MIMO three-node full-duplex network in the presence of a D2D wireless side channel. Our focus is to find out how the D2D wireless side channel will affect the fundamental tradeoff between efficiency and reliability of MIMO three-node network in the context of slow fading where the channel realizations though random, remain fixed over the communication period.
%
%We make the following contributions. Firstly, we obtain the optimal~(i.e., fundamental) DMT with channel state information known at the transmitter~(CSIT) for our proposed framework of side-channel assisted MIMO three-node network in its most general forms, allowing different multiplexing gains for UL and DL with arbitrary number of antennas at each node and channel parameters. We show that a vector bin-and-cancel~(BC) scheme involving a simple Han-Kobayashi message splitting, can achieve the optimal full-CSIT DMT with partial CSIT where only UL transmitter needs to be aware of the channel matrices of the interfering link. The No-side channel case is a special case incorporated in our framework, which improves upon half-duplex counterpart where the base station uses either time-division or frequency-division for UL and DL. We characterize the effect of the side channel on DMT, and quantify how the side channel bandwidth can help increase DMT over no-side-channel one. As expected, the DMT scales with the bandwidth of the side channel and can be maximized signifying that the system is no longer interference-limited.
%
%Secondly, we derive an achievable DMT~(i.e., a lower bound on the DMT) in the absent of CSIT for side-channel assisted MIMO three-node network.
%Under certain scenarios, we show analytically how the extra bandwidth of the side channel can compensate for CSIT, helping the no-CSIT DMT meet the optimal DMT with full-CSIT, thus establishing the optimal no-CSIT DMT. In the case where the number of transceiver antennas at the BS is larger than mobile nodes, we also show that the number of antennas at the BS is interchangeable with the extra side channel bandwidth for compensating CSIT.
%
%The rest of paper is organized as follows. Section 2 presents the system model.
%In Section 3, we derive the inner bound and outer bound of instaneous capacity region of the side-channel assisted MIMO three-node network.
%We show that a distributed full-duplex interference cancellation scheme named vector BC can achieve within a constant gap of the capacity region, which can be used to establish the optimal DMT of our system. Section 4 characterizes optimal DMT in its general form as an convex optimization problem, and we obtain the analytical solutions in several special cases. In Section 5, we find out the achievable DMT without CSIT, and characterize the effect of the side channel on DMT of the network.
%Section 6 concludes the paper.
%
%\emph{Notations:} We use $A^\dagger$ to denote Hermitian of $A$, and $|A|$ to denote the determinant of $A$. We use $(x)^+$ to denote the maximum of $x$ and 0. We use $\mathcal{CN}(0,Q)$ to denote a circularly symmetric complex Gaussian distribution with zero mean and covariance matrix $Q$. We use $\mathbf{I_{N}}$ to denote identity matrix of rank $N$. We use $f(x)\doteq g(x)$ to denote that $\lim_{x\rightarrow \infty}\frac{\mathrm{log}f(x)}{\mathrm{log}g(x)}=1$. We use $A\preceq B$ to denote that matrix $B-A$ is a positive-semidefinite positive~(p.s.d) matrix. For conciseness, we will use subscript 1 to denote DL channel, and subscript 2 to denote UL channel, superscript $s$ to denote D2D wireless side channel, and subscript 21 to denote INI link.
% We use $A\otimes B$ to denote the Kronecker product of matrix $A$ and $B$.


%\textcolor{red}{Jingwen, check the paper to use ``side-channel" not ``side channel"}

%% New Introduction
Increasingly, mobile devices have multiple radios to access different parts of the spectrum, e.g. cellular and ISM bands. The ability to access multiple parts of the spectrum simultaneously provides an opportunity to use multiple bands simultaneously in new and unique ways. A common method is to use the two bands simultaneously, to access both cellular and ISM band networks (notably WiFi) and is now an integral part of cellular provider data strategy to offload cellular traffic to WiFi networks~\cite{offload}. In this paper, we will consider the use of  device-to-device~(D2D) wireless channels between mobile devices, to serve as side-channels to \emph{aid} in the communication to the infrastructure nodes.
%The readily accessible wireless devices with multi-radio interfaces allows the use of multiple wireless bands simultaneously, which provides an opportunity to establish device-to-device~(D2D) wireless side channels when the mobiles are associated with the base station in the main channels.
For example, the main network could be on a cellular band while the D2D wireless side-channel could be on an unlicensed ISM band. We propose to use the ISM band side channel not for data off-loading, but for interference management in cellular bands, a scenario which we labeled as \emph{ISM-in-cellular} D2D side-channel~\cite{Jingwen,JingwenTWC}.
%Such D2D wireless side channels can be leveraged to facilitate main channel cellular communication.

Specifically, we will consider a three-node network, where the infrastructure node is full-duplex capable and is supporting a simultaneous uplink and downlink flow from two half-duplex mobiles as shown in Fig.~\ref{fig.1}.
Recent results on experimental evaluation of full-duplex wireless have demonstrated that short to medium range full-duplex communications (approaching 150 meters) is feasible with well designed infrastructure nodes ~\cite{Everett13Paper,duarte2012design}. Thus, we envision that the first use of full-duplex capabilities might be in small cell infrastructure~\cite{Smallcell}, supporting both full- and half-duplex mobile nodes.
%
% in short to medium ranges shows the feasibility of full-duplex wireless which greatly improve the spectral efficiency over its half-duplex counterpart, and opens new design opportunities for cellular wireless communication systems, such as small cells~\cite{Smallcell}.
\begin{figure}[h!]
  \centering
%\flushleft
%\flushright
    \includegraphics[width=0.35\textwidth,trim = 70mm
      50mm 65mm 35mm, clip]{pic/topology2.pdf}
  \caption{\emph{MIMO three-node full-duplex network: inter-node interference becomes an important factor when the full-duplex infrastructure node communicates with uplink and downlink mobile nodes simultaneously. }}
\label{fig.1}
\end{figure}

%\sout{With the above discussion as our backdrop, we consider the following three-node network shown in Fig.~\ref{fig.1}.}
In Fig.~\ref{fig.1},  the full-duplex capable base station~(BS) communicates with two half-duplex mobiles simultaneously to support one uplink~(UL) and one downlink~(DL) flow. One of the bottlenecks in this network is the inter-node interference from uplink mobile to downlink mobile node. In \cite{JingwenTWC}, we proposed a \emph{distributed full-duplex architecture} to leverage D2D side-channels to mitigate inter-node interference for the case when all nodes can only support single antenna (SISO) links. We note that our use of D2D link is different from its conventional use such as establishing peer-to-peer communication \cite{D2Doverlay}, forming virtual MIMO by cooperative communication \cite{D2Dvmimo} or offloading cellular traffic~\cite{D2Doffload}. In contrast, we propose to use the D2D side-channel only to mitigate the interference.%, and we study how to leverage the side-channel for advanced interference management to assist future wireless communication with full-duplex infrastructure node, which makes our work distinct from the rest.

%Our focus is to find out how the D2D wireless side channel will affect the fundamental tradeoff between efficiency and reliability of MIMO three-node network in the context of slow fading where the channel realizations though random, remain fixed over the communication period.

In this paper, we will study the MIMO three-node full-duplex network in the presence of a D2D wireless side-channel. Our driving question is if and how the spatial degree-of-freedom, i.e. number of antennas at the base station and mobiles, interact with the spectral degrees-of-freedom offered by the side-channel in slow fading channels. The diversity multiplexing tradeoff (DMT), introduced in \cite{DMTTse}, captures both spectral efficiency and reliability of a MIMO system experiencing slow fading in high signal-to-noise ratio~(SNR) limit. Thus, we analyze the optimal DMT of the general three-node MIMO case with a D2D side-channel under short term per-node constraint. We study two cases of channel state information -- channel state information only known at the receivers~(CSIR), and at both the receivers and the transmitters~(CSIRT). We compare the respective DMTs of the two cases to the upper bound of the system with no interference.

%Specifically, we study two scenarios of channel state information at the receiver~(CSIR) and at the transmitter~(CSIRT) which requires different system complexity since obtaining CSIT cost more operation overhead, thus allowing us to also understand the tradeoffs due to channel state information at the transmitter~(CSIT).

%Multiple-input multiple-output (MIMO) communication~\cite{biglieri2007mimo,stuber2004broadband,goldsmith2003capacity} is well-known to improve the spectral efficiency and reliability upon single-antenna case. The diversity multiplexing tradeoff (DMT), introduced in \cite{DMTTse}, captures both spectral efficiency and reliability of MIMO system in high signal-to-noise ratio~(SNR) limit. The DMT is also characterized for two-user interference channel~\cite{icdmt,icdmt2},
%%where each user can have different diversity and multiplexing gain requirement,
%and in \cite{DMTMIMOZ}, the optimal DMT is derived for MIMO Z-interference channel.
%The result of DMT is especially relevant in a slowly varying channel when the ergodic capacity may not be a meaningful metric.
Our findings are two-fold.

\note{The description of the results is still not very clear. We need to re-think it. I think the problem setup is too abstract. We need to state the problem with some variables clarified here - M1, N1, M2, N2, W.}

%\textcolor{red}{Jingwen, rewrite these two para and one way to state the main result as "We characterize the minimum bandwidth of the side channel required to achieve the upper bound on DMT, which corresponds to the case of no inter-device interference. When x < y, CSIRT outperforms CSIR by requiring less minimum bandwidth but x > y, there is no advantage to transmitter info. This is because.."}
First, we characterize the bandwidth of the side-channel required to compensate for channel state information at the transmitter~(CSIT) such that the DMT with CSIR matches the optimal DMT with CSIRT. We find out that the bandwidth required to bridge the gap due to CSIT is inversely proportional to the antenna resources at the base station. %The insights gained from the DMT analyses shed light on the spatial resources from multiple antenna  and the spectral resources from the side-channels.
\note{We need to give some insight into this reciprocal relationship.}

Second, we quantify the side-channel bandwidth required to achieve the no-interference upper bound, which is a function of antenna resources at mobiles. When the number of antennas at the uplink transmitter (UL in Fig.~\ref{fig.1}) is larger than that at the downlink receiver (DL in Fig.~\ref{fig.1}), the case of CSIRT outperforms that of CSIR by requiring less bandwidth to eliminate the effect of interference. However, when the number of antennas at the downlink receiver is larger than that at the uplink transmitter, there is no advantage of CSIT. The reason that the CSIT is not useful in the latter case is because the maximum multiplexing gain is limited by the uplink transmit antennas, therefore the receive beamforming at the interfered receiver together with the help of side-channel is sufficient to completely null out the interference.

%show that there is a clear correlation between antenna resources and the bandwidth of the side channel. We find out that a larger number of antennas at the interfered downlink receiver can result in spatial-spectral correlation for equal performance between the DMT of the system and the optimal DMT of point-to-point channels even without knowing CSIT. while a larger number of antennas at the interfering uplink transmitter only reveals the correlation between spatial degree-of-freedom and spectral degree-of-freedom under CSIRT assumption to completely eliminate the effect of interference.
%For example, in the CSIRT case, spatial degree-of-freedom at the mobile nodes are correlated one-to-one with spectral degree-of-freedom of the side channel for equal performance between the optimal DMT and point-to-point~(PTP) channels: larger number of antennas leads to less required side-channel bandwidth for nulling out interference. In CSIR case, the correlation  is that the side-channel bandwidth can be traded one-to-one with the number of antennas to completely compensate for CSIT such that the DMT with CSIR achieves the optimal DMT with CSITR.
%we study the case of multi-antennas mobiles. We find out that a larger number of antennas at the interfered DL receiver can result in spatial-spectral tradeoff for both CSITR and CSIR cases while a larger number of antennas at the interfering UL transmitter only reveals the tradeoff between spatial dof and spectral dof for CSITR case.
%Second, we show that a bulk of the complexity can lie in the base-station. We analyze the case of single-antenna mobiles with multiple antennas at the base station to quantify the spatial-spectral correlation between the side channel bandwidth and the antennas resources at the base station for equal
%performance between the DMT with CSIR and the optimal DMT with CSIRT such that the effect of CSIT can be eliminated completely.

To arrive at the above results, we derive the optimal DMT for CSIRT case and the DMT achieved for CSIR case. The expressions, due to their generality, are quite complex and only numerically solvable. However, one important case with \note{identical transmit and receive antennas - this is not clear - what do you mean by identical transmit and receive antennas?} at the base station is solved in closed form. We propose a vector bin-and-cancel scheme with a simple Han-Kobayashi~\cite{han1981new} message splitting, which achieves the the optimal DMT with CSIRT. We show that the gains due to leveraging the side-channel are significant, and increase with the side-channel bandwidth.

\note{Do we also propose/discuss the simpler schemes - decode/estimate-and-cancel? I think it will be good to include them if possible.}

%we derive the optimal DMT with channel state information known at the transmitter and receiver~(CSITR) for our proposed framework of side-channel assisted MIMO three-node network in its most general forms, allowing different multiplexing gains for UL and DL with arbitrary number of antennas at each node and channel parameters. We show that a vector bin-and-cancel~(BC) scheme involving a simple Han-Kobayashi message splitting, can achieve the optimal DMT with partial CSIT where only the UL transmitter needs to be aware of the channel matrices of the interfering link. We show that the DMT improvement due to the side channel is significant.

The rest of paper is organized as follows. Section 2 presents the system model.
In Section~3, we derive the inner and outer bound for instantaneous capacity region of the side-channel assisted MIMO three-node network.
We show that the vector bin-and-cancel scheme achieves within a constant gap of the capacity region, which can be used to establish the optimal DMT of our system. Section 4 gives the main theorems which characterize the general DMT for both CSIRT and CSIR cases. In Section 5, we study the tradeoff between spatial resources from multiple antennas and spectral resources of the side-channels on the symmetric DMT.
Section 6 concludes the paper.

\emph{Notations:} We use $A^\dagger$ to denote Hermitian of $A$, and $|A|$ to denote the determinant of $A$. We use $(x)^+$ to denote the maximum of $x$ and 0. We use $\mathcal{CN}(0,Q)$ to denote a circularly symmetric complex Gaussian distribution with zero mean and covariance matrix $Q$. We use ${I_{N}}$ to denote identity matrix of rank $N$. We use $f(x)\doteq g(x)$ to denote that $\lim_{x\rightarrow \infty}\frac{\mathrm{log}f(x)}{\mathrm{log}g(x)}=1$. We use $A\preceq B$ to denote that matrix $B-A$ is a positive-semidefinite positive~(p.s.d) matrix. For conciseness, we will use subscript dl to denote downlink channel, and subscript ul to denote uplink channel, superscript S to denote D2D wireless side-channel, and subscript I to denote inter-node interference channel. 

==> SpecialCase3.tex <==
% !TEX root = TITSidechannel.tex

\section{Spatial and Spectral Tradeoff in DMT}
In this section, we will derive the optimal DMT in closed form for the case when the base station has equal number of transmit and receive antennas~(i.e, $M_{\mathrm{dl}}=N_{\mathrm{ul}}=M$) in symmetric channels. Using the closed-form DMT expressions, we will compare three systems: (i) the side-channel assisted three-node network with CSIRT, (ii) the side-channel assisted three-node network with CSIR, and (iii) an idealized three-node network without interference, i.e., a parallel uplink and a downlink channel; the last network provides us the benchmark for best possible performance.  By comparing these three networks, we aim to quantify the interplay between the spatial resources of multiple antennas and spectral resources of the side-channel.
%we will derive the  bandwidth of the side-channel such that system DMT matches that of a system with no interference.

%Often in practical wireless communication systems, the base station in a cellular network can host more antennas compared to space-constrained mobile nodes.

%In this section, we will compare the DMT of three systems: (i) the side-channel assisted three-node network with CSIRT, (ii) the side-channel assisted with only CSIR, and (iii) is two parallel uplink and downlink channels, i.e., the three-node network without interference.

%We define the \emph{essential bandwidth} as the bandwidth ratio to eliminate the effect of interference such that the system with either CSIRT or CSIR will achieve the same performance as point-to-point channel. As a byproduct, we will also study the \emph{minimum bandwidth} as the bandwidth ratio of the side-channel to main channel to eliminate the effect of CSIT such that the system with CSIR achieves the same performance as the system with CSIRT.
\subsection{Main Results}
We assume the full-duplex capable base station has $M$ transmit and receive antennas, respectively. Recall that the uplink mobile has $M_{\mathrm{ul}}$ transmit antennas and downlink mobile has $N_{\mathrm{dl}}$ receive antennas. We assume that $M\geq M_{\mathrm{ul}},~ N_{\mathrm{dl}}$.
We first present the closed-form symmetric DMT of $(M,N_{\mathrm{dl}},M_{\mathrm{ul}},M)$ system with $\alpha_{\mathrm{dl}}=\alpha_{\mathrm{ul}}=\alpha_{\mathrm{I}}=1$ and $r_{\mathrm{dl}}=r_{\mathrm{ul}}=r$ under CSIRT and CSIR assumptions in  Lemma~\ref{case3} and Lemma~\ref{case33}, respectively.

With the lemmas above, first we ask the question that how much side-channel bandwidth is required to eliminate the effect due to CSIT such that the DMT of the system with CSIR matches that of the system with CSIRT, which can be quantified in the following theorem.
\begin{theorem} \label{coro1}
In case of $(M,N_{\mathrm{dl}},M_{\mathrm{ul}},M)$, we give the sufficient condition where the lack of CSIT can be compensated such that the DMT without CSIT reaches the optimal DMT with CSIT
\begin{enumerate}
  \item
$W =\min\left\{\frac{N_{\mathrm{dl}}+M_{\mathrm{ul}}-1}{M+N_{\mathrm{dl}}-M_{\mathrm{ul}}+1}, \frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{N_{\mathrm{dl}}}{M_{\mathrm{ul}}}\right)^+\right\} ~\text{where}~\alpha_{\mathrm{S}}\!\geq\!\frac{d_{M,M_{\mathrm{ul}}}\left(\frac{M_{\mathrm{ul}}}{2}\right)\!-\!M(N_{\mathrm{dl}}\!-\!M_{\mathrm{ul}})}{M_{\mathrm{ul}}N_{\mathrm{dl}}},$  when $N_{\mathrm{dl}}\geq M_{\mathrm{ul}},~M_{\mathrm{ul}}=1, 2$;
 % $W\!=\!\min\left\{\frac{N_{\mathrm{dl}}+M_{\mathrm{ul}}-1}{M+N_{\mathrm{dl}}-M_{\mathrm{ul}}+1}, \frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{N_{\mathrm{dl}}}{M_{\mathrm{ul}}}\right)^+\!\right\}$ for $M_{\mathrm{ul}}=1$
  %or $W\!=\!\min\left\{\frac{N_{\mathrm{dl}}+M_{\mathrm{ul}}-1}{M-N_{\mathrm{dl}}+1},\frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{N_{\mathrm{dl}}}{M_{\mathrm{ul}}}\right)^+\!\right\}$ for $N_{\mathrm{dl}}\!\geq\! M_{\mathrm{ul}}$, when $\alpha_{\mathrm{S}}\!\geq\!\frac{d_{M,M_{\mathrm{ul}}}\left(\frac{M_{\mathrm{ul}}}{2}\right)\!-\!M(N_{\mathrm{dl}}\!-\!M_{\mathrm{ul}})}{M_{\mathrm{ul}}N_{\mathrm{dl}}}$;
  \item $W=0,$ when $N_{\mathrm{dl}}\geq \frac{d_{M_{\mathrm{ul}},M}\left(\frac{M_{\mathrm{ul}}}{2}\right)}{M}+M_{\mathrm{ul}},~M_{\mathrm{ul}}=1,2$.\label{w0}
\end{enumerate}
\end{theorem}
\begin{proof}
We only need to compare the symmetric DMT with CSIRT in Lemma~\ref{case3} and that with CSIR in Lemma~\ref{case33} to find out the condition where their expressions are the same.
\end{proof}
\begin{corollary}\label{coro5}
When $M_{\mathrm{ul}}> N_{\mathrm{dl}}$, if $W<\frac{1}{\alpha_{\mathrm{S}}}$, the DMT with CSIR is strictly smaller than that with CSIRT.
\end{corollary}

Corollary~\ref{coro5} can be readily obtained from Lemma~\ref{case3} and Lemma~\ref{case33}. If $M_{\mathrm{ul}}> N_{\mathrm{dl}}$, the availability of CSIT will play a role in performing transmit beamforming. Meanwhile, if $W<\frac{1}{\alpha_{\mathrm{S}}}$, namely, the side-channel could not completely help eliminate the interference, the maximum multiplexing gain  with CSIR will be strictly smaller than that with CSIRT.

The next question we will ask is how much side-channel bandwidth is required to eliminate the effect of interference such that the DMT of the system with either CSIRT or CSIR matches that with no-interference upper bound. The following theorem characterizes the effect of the side-channel bandwidth on the performance of the symmetric DMT.
\begin{theorem}\label{coro3}
In case of $(M,N_{\mathrm{dl}},M_{\mathrm{ul}},M)$, we given the sufficient condition where the effect of interference can be completely eliminated such that the DMT with/without~(w/wo) achieves the PTP performance
\begin{enumerate}
\item
$W_{\text{CSIT}}=\frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{m_X}{m_{\rm I}}\right)^+, \alpha_{\mathrm{S}}\!\geq\!\frac{(2m_{\rm I}-m_X)(M-m_{\rm I}+1)}{m_{\rm I}(2|N_{\mathrm{dl}}-M_{\mathrm{ul}}|+2)}.$
\item
\[
W_{\text{No~CSIT}}=\left\{
  \begin{array}{l l}
  \frac{1}{\alpha_{\mathrm{S}}}, \alpha_{\mathrm{S}}\geq\frac{M-N_{\mathrm{dl}}+1}{2(M_{\mathrm{ul}}-N_{\mathrm{dl}}+1)}, ~\text{when}~M_{\mathrm{ul}}\geq N_{\mathrm{dl}}\\
  \frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{m_X}{m_{\rm I}}\right)^+,\alpha_{\mathrm{S}}\!\geq\!\frac{(2m_{\rm I}-m_X)(M-m_{\rm I}+1)}{m_{\rm I}(2|N_{\mathrm{dl}}-M_{\mathrm{ul}}|+2)},~\text{when}~  N_{\mathrm{dl}}\geq M_{\mathrm{ul}}
   \end{array} \right.
   \]
\end{enumerate}
\end{theorem}
\begin{proof}
We need to only from the special structure of the the decay slope of the piecewise linear function $d_{M,N}(r)$ diminishes in each subfunction as $k$ increases. For $r\in[k-1,k]$, where $k\in[1,\min(M,N)]$ is an integer. The decay slope is $(M+N-2k+1)$,  Thus we only need compare the decay slope of the last piece of function $d_{\rm sum}$ with $d_{\rm PTP}$.
We need to compare the optimal DMT with CSIRT in Lemma~\ref{case3} and the DMT achieved with CSIR in Lemma~\ref{case33} with the optimal DMT of point-to-point channel. When $M_{\mathrm{ul}}\geq N_{\mathrm{dl}}$, we can show that if the bandwidth ratio in CSIRT case satisfies that $W_{\mathrm{CSIRT}}= \frac{1}{\alpha_{\mathrm{S}}}\left(2-\frac{M_{\mathrm{ul}}}{N_{\mathrm{dl}}}\right)^+$, for $\alpha_{\mathrm{S}}\geq\frac{d_{N_{\mathrm{dl}},M}\left(\frac{M_{\mathrm{ul}}}{2}\right)}{M_{\mathrm{ul}}N_{\mathrm{dl}}}$, the DMT is dominated by the single-user performance for any $r\leq N_{\mathrm{dl}}$. Likewise, we can derive $W_{\rm{CSIR}}$ for CSIR case.
When $N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$, we can also find out that by satisfying the conditions given above, the DMT is dominated by the single-user performance.
\end{proof}
\subsection{Discussion of the Results}
Fig.~\ref{fig} illustrates the comparison of the three systems as a function of the side-channel bandwidth. When $N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$, there are three regimes in comparison of DMT performance. In the first regime, the performance of CSIR is worse than that of CSIRT. In the second regime, when $W$ is greater than a threshold, CSIT is of no use. The DMT is first determined by the single-user performance~(either downlink or uplink mobile user); then there are two types of dominant error events, one is that users in the side-channel are in error and the other one is that after performing receive beamforming all users are in error, both of which lead to the same DMT with/without~(w/wo) CSIT. In the last regime, the use of side-channel will completely cancel out the interference such that the dominant error event is that only one user is in error. On the other hand, when $M_{\mathrm{ul}}> N_{\mathrm{dl}}$, the availability of CSIT always provides an additional gain for performing transmit beamforming. Also, with CSIT less side-channel bandwidth is required to meet the no-interference upper bound. Note that the strength of the side-channel level $\alpha_{\mathrm{S}}$ is implicitly incorporated in Theorems~\ref{coro1} and \ref{coro3}, thus is omitted in Fig.~\ref{fig}.

\begin{figure}
\centering
\subfigure[$N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$]{\scalebox{0.62}{\input{pic/n1gm22.pdftex_t}}\label{fig:subfig2}}
\hspace{0.6cm}
\subfigure[$M_{\mathrm{ul}}> N_{\mathrm{dl}}$]{\scalebox{0.62}{\input{pic/m2gn1.pdftex_t}}\label{fig:subfig1}}
\caption{Comparison of the three systems as a function of the side-channel bandwidth.}\label{fig}
\end{figure}

In the following section, we will further elucidate the results for single-antenna mobiles and multiple-antenna mobiles cases, respectively.
%\subsubsection{Single-antenna Mobiles}
%In Fig.~\ref{Spectral}, we first show the symmetric DMT w/wo side-channel and w/wo CSIT when $\alpha_{\mathrm{dl}}=\alpha_{\mathrm{ul}}=\alpha_{\mathrm{I}}=\alpha_{\mathrm{S}}=1$ in SISO channel. The no-side-channel case in~\cite{sezgin2009diversity} is a special case incorporated in our derivation of DMT. From Fig.~\ref{Spectral}, we can see that in the three-node network, the full-duplex capable base station is always superior to its half-duplex counterpart where the base station adopts either time-division multiplexing~(TDM) or frequency-division multiplexing (FDM) for uplink and downlink. We also observe that increasing bandwidth ratio will improve the maximum multiplexing gain. Meanwhile, given the symmetric multiplexing gain, larger bandwidth ratio will render higher diversity order. Specifically, when $W\geq\frac{1}{2}$, the lack of CSIT will be compensated such that the DMT with CSIR and CSIRT have equal performance; when $W\geq1$, the DMT of the system w/wo CSIT will be maximized to achieve no-interference performance.
%\begin{figure}[h!]
%  \centering
%%\flushleft
%%\flushright
%    \includegraphics[width=0.4\textwidth,trim = 65mm
%      50mm 75mm 45mm, clip]{pic/SISOspecial.pdf}
%  \caption{Symmetric DMT for both CSIRT and CSIR when $\alpha_{\mathrm{dl}}=\alpha_{\mathrm{ul}}=\alpha_{\mathrm{I}}=\alpha_{\mathrm{S}}=1$ in SISO channel.}
%\label{Spectral}
%\end{figure}

When both the uplink and downlink mobiles are equipped with single-antenna,  %and Theorem~\ref{coro3}, we can obtain that
%\begin{corollary}\label{coro51}
%When $M_{\mathrm{ul}}=N_{\mathrm{dl}}=1$, if the side-channel bandwidth ratio satisfies that $W=\min\left\{\frac{1}{M+1},\frac{1}{\alpha_{\mathrm{I}}^s}\right\},~\text{where}~ \alpha_{\mathrm{I}}^s\geq \frac{M}{2}$,  the DMT with CSIR achieve the same performance as that with CSIRT;
%\end{corollary}
from Theorem~\ref{coro1}, we can conclude that in order to eliminate the effect of CSIT, it is sufficient if the side-channel condition captured by the product $W\alpha_{\mathrm{S}}$ satisfies that $W\alpha_{\mathrm{S}}\in\left[\frac{1}{4},\frac{1}{2}\right)$ with $W\geq \frac{1}{M+1}$ and $\alpha_{\mathrm{S}}\geq \frac{M}{2}$.
Fig.~\ref{sst1} illustrates the side-channel bandwidth required to compensate for CSIT as stated in Theorem~\ref{coro1} with single-antenna mobiles. We find  that the side-channel bandwidth for compensation of CSIT is inversely proportional to the antenna resources at the base station. The caveat is that the side-channel level $\alpha_{\mathrm{S}}$, on the other hand, has to grow with increasing number of antennas at the base station.
\begin{figure}[h!]
  \centering
%\flushleft
%\flushright
    \includegraphics[width=0.33\textwidth,trim = 30mm
      90mm 42mm 95mm, clip]{pic/sst1.pdf}
  \caption{The required bandwidth ratio to compensate for CSIT as a function of the number of antennas at the base station with single-antenna mobiles when $\alpha_{\mathrm{S}}=\frac{M}{2}$.}
\label{sst1}
\end{figure}


To understand the result above, let us look at the decaying slope of DMT for different channels in the three-node network. The decaying slope of the multiple access channel~(MAC) in the three-node network is $M+1$, while the the decaying slope of the side-channel is $\frac{1}{W}$. Therefore if $W\geq \frac{1}{M+1}$, the users in MAC will first be in error followed by the users' error event in the side-channel. When there is no side-channel available, the diversity gain drops to zero w/wo CSIT when $r=\frac{1}{2}$. However, with the help of side-channel, the diversity gain can be boosted to $\alpha_{\mathrm{S}}$. If $\alpha_{\mathrm{S}}\geq \frac{M}{2}$, the error event in the three-node network with or without CSIT is dominated by single-user performance when the symmetric multiplexing gain\footnote{For point-to-point channel, the diversity gain is $\frac{M}{2}$ when $r= \frac{1}{2}$.}  $r\leq \frac{1}{2}$. When $r\geq \frac{1}{2}$, the dominant error event is determined by the performance of the users in the side-channel, which is the same for both CSIR and CSIRT cases.\footnote{Note that the DMT of MAC channel with CSIR is different from that with CSIRT.}


In order to eliminate the effect of interference such that the DMT with or without CSIT achieve no-interference upper bound, it is both necessary and sufficient if the side-channel condition satisfies that $W\alpha_{\mathrm{S}}\geq 1$ according to Theorem~\ref{coro3}. Hence the required side-channel bandwidth is inversely proportional to the strength of the side-channel as to null out the interference.
The implication of such result is that in a highly clustered urban scenario, when the mobile devices are close to each other indicating higher side-channel strength, less side-channel bandwidth is required to completely cancel out the inter-node interference.
\subsubsection{Multiple-antenna Mobiles}
Fig.~\ref{MIMO1} shows the DMT in the absence of the side-channel when both the mobiles have multiple antennas. First, we can find out that in the three-node network, the gains due to the full-duplex capable base station over its half-duplex counterpart which do not utilize either CSIR or CSIT is particularly larger for MIMO channels compared to the SISO case in Fig.~\ref{Spectral}.
Second, a larger number of downlink receive antennas can also completely eliminate the effect of CSIT such that the DMT with CSIR achieves the optimal DMT with CSIRT as stated in Theorem~\ref{coro1}. For example, the DMT of $(3,3,2,3)$ with CSIR has the same performance as that with CSIRT. While in the case of $(3,2,3,3)$, the lack of CSIT will result in significant loss. Moreover, from Lemma~\ref{case3} and Lemma~\ref{case33} by substituting $W=0,\alpha_{\mathrm{S}}=0$, we can find out that when $N_{\mathrm{dl}}> M_{\mathrm{ul}}$, the maximum multiplexing gain with CSIR is the same as that with CSIRT, while for $M_{\mathrm{ul}}> N_{\mathrm{dl}}$, lacking CSIT will always cause a strictly smaller maximum multiplexing gain.
%\begin{figure}[h!]
%\begin{minipage}[b]{0.5\linewidth}
%  \centering
%%\flushleft
%%\flushright
%     \scalebox{0.4}{\includegraphics[trim = 50mm
%      45mm 28mm 40mm, clip]{pic/MIMOspecial1.pdf}}
%  \caption{The symmetric DMT of three-node full-duplex network without side-channel for $\alpha_{\mathrm{dl}}=\alpha_{\mathrm{ul}}=\alpha_{\mathrm{I}}=1$.}
%\label{MIMO1}
%\end{minipage}
%\hspace{0.1cm}
%\begin{minipage}[b]{0.4\linewidth}
%  \centering
%%\flushleft
%%\flushright
%    \scalebox{0.4}{\includegraphics[trim = 50mm
%      45mm 40mm 45mm, clip]{pic/MIMOspecial2.pdf}}
%  \caption{The symmetric DMT with side-channel for $\alpha_{\mathrm{dl}}=\alpha_{\mathrm{ul}}=\alpha_{\mathrm{I}}=\alpha_{\mathrm{S}}=1$.}
%\label{MIMO}
%\end{minipage}
%\end{figure}

Comparing Fig.~\ref{MIMO1} and Fig.~\ref{MIMO}, we can quantify the gains due to the extra side-channel bandwidth, which is significant especially in MIMO. In the case of $(3,2,3,3)$ when the system is lightly loaded, for instance, $r\leq 2/3$, there is no additional gain due to CSIT or $r\leq 5/4$, there is no gain due to the side-channel since the error event is dominated by point-to-point performance. Beyond those points, the dominant error event is that all users are in error, thus leveraging the CSIT or side-channel to perform vector bin-and-cancel will reduce the probability that such outage event happens.
%\subsection{Spatial-spectral Correlation with single-antenna Mobiles}

From Theorem~\ref{coro3}, we conclude that with CSIRT, as the antenna number ratio $\frac{\max\{M_{\mathrm{ul}},N_{\mathrm{dl}}\}}{\min\{M_{\mathrm{ul}},N_{\mathrm{dl}}\}}$ increases, the side-channel bandwidth required to completely eliminate the effect of interference reduces. Fig.~\ref{sst2} shows the required bandwidth to eliminate the interference as a function of antenna resources at mobiles when $N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$. In particular, if the antenna number ratio $\frac{\max\{M_{\mathrm{ul}},N_{\mathrm{dl}}\}}{\min\{M_{\mathrm{ul}},N_{\mathrm{dl}}\}}=2$, then we do not need to leverage the side-channel to achieve the interference-free performance.
Hence the spatial resources
of the multiple antennas at transmitters and receivers is
interchangeable with the spectral resources of the side-channel
bandwidth to cancel out interference. The intuition behind such spatial and spectral tradeoff is that the spatial degree-of-freedom at the mobiles for transmit/receiver beamforming is equivalent to the spectral degree-of-freedom of the side-channel for vector bin-and-cancel as to eliminate the interference completely.
%\end{remark}
%\begin{figure}[h!]
%  \centering
%%\flushleft
%%\flushright
%    \includegraphics[width=0.33\textwidth,trim = 30mm
%     90mm 43mm 95mm, clip]{pic/sst2.pdf}
%  \caption{The required bandwidth ratio for elimination of interference as a function of the antennas resources at mobiles, when $N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$ and $\alpha_{\mathrm{S}}=1$.}
%\label{sst2}
%\end{figure}

Second, we infer that Theorem~\ref{coro3} that when $M_{\mathrm{ul}}\geq N_{\mathrm{dl}}$, the system with CSIRT always outperforms that with CSIR by requiring less side-channel bandwidth to eliminate the interference.~\footnote{The system with CSIRT also has a weaker requirement of the strength of the side-channel level compare to that with CSIR.} However, when $N_{\mathrm{dl}}\geq M_{\mathrm{ul}}$, there is no advantage due to CSIT in certain regimes. Thus we can conclude that the more spatial degree-of-freedom at the interfered downlink receiver or side-channel bandwidth can simplify transceiver design by ruling out the necessity of obtaining CSIT to achieve the no-interference upper bound.

%The intuition behind such results is that with a larger number of antennas at the downlink receiver, the degree-of-freedom of the system~(maximum multiplexing gain) is limited by the interfering uplink transmit antennas, therefore only the interfered receiver need to perform receive beamforming to null out the interference.
%\end{remark}
%If the bandwidth ratio $W\geq 1$ for $\varphi=1$, the DMT with CSIR will also achieve PTP performance for multi-antennas mobiles, which matches the result for single-antenna mobiles case as stated in Corollary~\ref{coro2}. \vdots

%The reason behind above results can be understood as follows. The role of CSIT is to enable the uplink transmitter to send its data in the orthogonal space of the downlink signal space. And the role of the side-channel is to send message in the orthogonal spectral space of the main channel for interference cancellation. A larger number of interfered receive antennas can perform receive beamforming to null out the interference. Therefore the side-channel bandwidth is correlated with antenna resources at downlink mobile to achieve equal performance with or without CSIT. Moreover, increasing the bandwidth of side-channel or antennas at mobiles to perform transmit/receive beamforming will completely eliminate the effect of interference, which yields a correlation between the side-channel bandwidth and antenna resources to achieve the best performance without interference.
%Fig.~\ref{sst1} shows the minimum bandwidth of the system with CSIR as a function of the number of antennas at the base station for single-antenna mobiles. %The available spatial degree-of-freedom at the base station and provides
%\begin{figure}[h!]
%  \centering
%%\flushleft
%%\flushright
%    \includegraphics[width=0.38\textwidth,trim = 30mm
%      90mm 42mm 95mm, clip]{pic/sst1.pdf}
%  \caption{The minimum bandwidth of the system with CSIR as a function of the number of antennas at the base station with single-antenna mobiles.}
%\label{sst1}
%\end{figure}
%\begin{remark}
%
%%\textcolor{red}{Jingwen, I don't understand this para.}
%%The extra side-channel bandwidth is interchangeable with the number of antennas at the base station to eliminate the effect of CSIT. Namely, when the side-channel level increases with $M$ such that $\alpha^s_{21}\geq\frac{M}{2}$, if we have more antennas equipped at the base station, then we can leverage less side-channel bandwidth to bridge the gap due to CSIT such that the DMT with CSIR achieves the optimal DMT with CSIRT. Moreover, if $W\alpha^s_{21}\geq 1$, then the DMT of the system w/wo CSIT can also achieve point-to-point performance to eliminate the effect of interference.
%We show the minimum bandwidth of the bandwidth region stated in Theorem~\ref{coro1}. We find out that the minimum bandwidth is inversely proportional to the antenna resources at the base station. Since a bulk of the complexity can lie in the base station, the required bandwidth of the side-channel will be very small with large number of antennas at the base station, which is shown in Fig.~\ref{sst1} with single-antenna mobiles.
%\begin{figure}[h!]
%  \centering
%%\flushleft
%%\flushright
%    \includegraphics[width=0.4\textwidth,trim = 65mm
%      50mm 75mm 45mm, clip]{pic/SISOspecial.pdf}
%  \caption{Symmetric DMT for both CSIRT and CSIR when $\alpha_{1}=\alpha_{2}=\alpha_{21}=\alpha^s_{21}=1$ in SISO channel.}
%\label{Spectral}
%\end{figure}
%%The reason behind such results is that the maximum multiplexing gain is limited by the single antenna mobiles. A larger number of antennas at the base station can improve the diversity order at given symmetric multiplexing gain $r$. Also, the bandwidth of side channel helps increase diversity order only. Therefore the side channel bandwidth is correlated with number of antennas at the base station for achieving equal performance w/wo CSIT.
%
%We also show the symmetric DMT w/wo side-channel and w/wo CSIT for SISO in Fig.~\ref{Spectral}. Note that the no-side-channel case in~\cite{sezgin2009diversity} is a special case incorporated in our derivation of DMT. And increasing bandwidth ratio will improve the maximum multiplexing gain. Specifically, when $W\geq\frac{1}{2}$, the lack of CSIT will be compensated such that the DMT with CSIR and CSIRT have equal performance; when $W\geq1$, the DMT of the system will be maximized to achieve point-to-point performance.
%The multiple antennas at the base station thus can be leveraged to alleviate interference
%\end{remark}
%\begin{remark}
%The no side-channel special case is incorporated in our derivation of DMT, which improves upon the half-duplex~(HD) counterpart where the base station uses either time-division multiplexing~(TDM) or frequency-division multiplexing (FDM) for UL and DL as shown in Figure~\ref{Spectral}. This is because TDM/FDM is just among all the achievable schemes captured by our framework of side-channel assisted MIMO three-node network when $W=0$.
%\end{remark}

